Covert Association of Applications on Edge Devices by Processor Workload

The scheme of application (app) distribution systems involving incentivized third-party app vendors is a desirable option for the emerging edge computing systems. However, such a scheme also brings various security challenges as faced by the current mobile app distribution systems. In this paper, we study a threat named covert device association, in which the vendors of two apps collude to figure out which of their app installations run on the same edge device. If the two colluding apps are popular, the threat can be used to launch various types of further attacks at scale. For example, the user of the compromised edge device, who wishes to remain anonymous to one of the two apps, will be de-anonymized if the user is not anonymous to the other app. Moreover, the coalition of the two apps will have an escalated privilege set that is the union of their individual privilege sets. In this paper, we implement the threat by a reliable and ubiquitous covert channel based on the edge device processor workload. The implementations on three edge devices (two smartphones and an embedded compute board) running Android and Android Things do not require any privileged permissions. Our implementations cover three attack scenarios of 1) two apps running on the same Android phone, 2) an app and a web session in the Tor browser running on the same Android phone, and 3) two apps running on the same Android Things device. Experiments show that the covert channel gives at least 0.25 bps data rate and the covert device association takes at most 3.2 minutes.

==> main_appendices.tex <==


% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%


\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.


% use section* for acknowledgment
\section*{Acknowledgment}


The authors would like to thank...



==> sec_approach.tex <==
\section{Implementation Principal}
In this section, we present the feasibility and throughput of communication using the total CPU load in two Android-based operating systems that Android Phone OS and Android things OS. Because we utilize the same set of theoretical knowledge in the two operating systems mentioned above, we divide our experimental object into two sections(Android Phone section, IoT device section). The general idea is that the Sender runs the malicious software to send a message; the Receiver monitors the CPU load on all cores continuously to receive the message. Throughout, we refer to the total CPU load as CPU load rather than the running situation for a special core, the information we transmit is binary by default, and the phone refers to the smartphone with the Android operating system. First, we describe our experimental setup.


\subsection{Experimental Setup}
We base our analysis on experimental data collected from two common and representative devices:
\subsubsection{}
a Xiaomi/ Redmi 2 4G Dual SIM including 4x ARM Cortex-A53 processors, intalls 5.1.1 Android Version.The max frequency is clocked at 1.2GHZ. 

\subsubsection{}
a Raspberry Pi 3 Model B, 16GB Micro SD Card with NOOBS, featuring a quad-core ARM8 processor clocked at 1.2MHZ;

In the rest of the paper, we refer to the device 1 as  Android phone and the device 2 as loT device. Android phone is representative of the current hand-held Android smartphone; IoT device is representative of devices which include an SoM, carrier board, and peripherals(NXP Pico i.MX7D and Raspberry Pi 3 Model B). Using this setup, we achieve the covert channel by running programs in these two platforms and analyze the channels for capacity estimation and evaluate a communication scheme.
\subsection{Covert Communication in Android phone}
This section illustrates the process from acquiring the CPU load in two distinct methods to the running programs to influence the magnitude of CPU load. If the Sender and the Receiver share a specific communication protocol, some important information can be leaked by detecting continuously the variation of the CPU load which could cause severe security problems.

\subsubsection{Acquiring CPU load situation}

We think using the total CPU load is a perfect way to construct a covert channel. Because we straightly alter the total CPU demanding rather than paying attention to process distribution in different cores or CPU affinity... Without loss of generality, we use two methods to reflect the total CPU load situation, instant total CPU load, and instant CPU frequency. As for the former one, the total CPU load represents a measure of all CPU running demand over a specific period of time. As for the letter, based on CPU frequency scaling technology, we calculate one value to reflect total CPU demanding situation using CPU frequency and we call it Load Frequency Ratio, reported in Equation(1).\\\rule[-10pt]{9cm}{0.05em}\begin{align*}
    Y=\sum_{i=1}^{n} 1/n*(Fre_i/FreMAX_i) && \text{Equation (1)}\\ 
    \text{Y is the Load Frequency Ratio}\\
    \text{n is the number of device cores}\\
    \text{Fre is the frequncy of current core}\\
    \text{FreMAX is the max frequncy of current core}   
\end{align*}\rule[-10pt]{9cm}{0.05em} It also could reflect total CPU running demand during a specific period time. Because there is a feature in Android (via the Linux kernel) which allows the clock frequency of the processor to be varied, scaled-down when the phone is not being used much and ramped up when needed. As you know, a mobile system needs to be tuned to save as much power as possible yet while offering the best performance available. So we have seized on this character, which means getting the frequency of the start time and finish time in a period we could indirectly know the busyness of CPU.

 
We read the CPU load in proc/stat file in that proc file system provides detailed information about kernel, processes, and configuration parameters and we read CPU frequency in /sys/devices/system/cpu/cpu */cpufreq file.

 
Due to the old Android version, our Android phone can easily read the CPU load from proc/stat file. However, On December 5, 2017, Google officially released Android 8.1, the main update for Android Oreo. Android O further reduces access to the /proc filesystem relative to Android N by removing access to the "stat" pseudo-file by its SELinux configuration. Even we couldn't read proc file in the latest Android version but there still are some other methods to get CPU load(top command, Time assembly instruction) while getting CPU frequency is still easy. The key point of this paper doesn't deliberate how to attain CPU load and CPU frequency without any trouble. Because the function of human-computer interaction of phones is more and more popular, some system information will still be obtained in order to realize these functions. To offer better user service Google impossible ban all APIs and there are many other ways to obtain these values somehow. Based on these theories, we can achieve Receiver.

Receiver: The purpose of the Receiver is to collect the information of the CPU load during the data transmission in a certain sampling frequency. According to the two methods of acquiring the CPU load. we also create one APP to acquire CPU load synchronously. Without the complex function of the Sender, this APP only needs to realize synchronization with the Sender and record the instant temperature of the battery. As for the sampling rate, our sampling mechanism bases on Nyquist Sampling Theorem. In our experiment, the sampling rate is four times faster than that of Sender APP which is a basic requirement to recover the original signal. Every time we save the acquired CPU information into the CSV file on the phone.

\subsubsection{Encoding the waveform to send information}

For a complete communication system, we need these basic elements: the Sender, the message, the Receiver, the medium channel. We assume that the information that needs to be transmitted is a series of binary numbers and we have also proposed about the Receiver(acquiring CPU load). This section illustrates the method to fulfill Sender.


To successfully send our information, Sender is a crucial component which drives specific CPU waveform to transmit our information. As part of digital communications, we choose Amplitude-shift keying (ASK) and Frequency-shift keying (FSK) as our communication methods. Unipolar non-return-to-zero code is our code pattern for ASK which means the upper CPU load represents the number 1 in a certain period, and the lower CPU load means the number 0. No matter sending number 1 or 0, it share the same period for one bit. As for FSK which sends information through frequency changes of the carrier signal, We directly use ASK as our carrier signal. In the same period for one bit, continuous five times wave 1 and wave 0, what is mentioned in ASK before, represents the number 1, and once wave 1 and wave 0 represents number 0.

Sender: We aim to design an Android APP to convert the information into the previously mentioned communication code pattern. We know that it is very easy to affect the CPU load like the infinite loop, but too much load will cause the phone to heat up and get stuck or some severe situations, so how to accurately generate the CPU load becomes our first task. As we know, Different mobile phone's CPU models and core numbers are not identical. So The test load depends on the core numbers. In more detail, we use the Threadpool of JAVA to open (core number -2) threads, and each thread will do the repetitive operation or sleep operation according to the value of the transmission information. In this way, the CPU waveform could secretly transmit some information.

Now that the basic part of the communication system has been established, a reasonable experiment should be established to verify its potential. First, we have to address the problem of synchronization between Sender and Receiver. On account of that the two parts of the java code are not very prolix, we integrated it into the same APP and started the communication with a button that would start all programs at the same time. It is convenient to test our Sender in this way rather than opening two APPs.

For Phone APP, the user's operation on the device must cause changes in the CPU load, and these unavoidable changes are noise in the channel. So we decide to divide the experiment into two parts, one that runs our program without any interference, and two that always play the movie during the data transmission as interference. 

\subsection{Covert Communication in IoT devices}

This section we illustrate the communication realization in IoT devices. The advent of the IoT is one of the most dynamic and exciting developments in information and communications technology. Based on the development of Android phones, we decided to use Android Things as our operating system of IoT devices. Moreover, Google emphasizes that developers are able to use familiar Android SDKs, APIs, and services including the Google Cloud Platform. So Android Things' CPU load acquisition and information transmission by changing CPU load waveform are the same as mobile phones B).  The focus of our discussion will be on the features of Android Things and experimental details.
\subsubsection{Features of Android Things}

Android Things is an Android-based embedded operating system platform by Google, announced at Google I/O 2015. It is aimed to be used with low-power and memory-constrained IoT devices, which are usually built from different MCU platforms. Where Android Things differs from normal Android is that it can control peripherals and read sensors. Anything from temperature sensors through LCDs and on to servo motors can be used by Android Things. This interaction is done via the General Purpose Input Output (GPIO) ports which you find on boards like the Raspberry Pi. Google once used a sentence to describe Android Things: If you can build an app, you can build a device.

\subsubsection{Experimental details}

First, since Google does not prevent access to the hardware information as much as phones, we just read the CPU load from proc/stat to get the data. To explore the potential of this communication method in IoT devices, we still transmit information by ASK, FSK using CPU load and the sampling rate of the Receiver program is four times faster than that of the Sender program. Of course, we integrate these two parts into one APP like phone and running it in two situations, without interference, having interference. As for the interference situation, We create a script that allows the device to decompress a file continuously during the information transfer process.
\subsection{Experimental setting and related problems}
According to the illustration of B) and C), it is clear how load-based communication works between mobile phones and IoT devices. Then we present the experimental setting and related problems. 
\subsubsection{Experimental setting}

For the sake of judging the advantages and disadvantages of data transmission, We need to experiment with different baud rates which could be used to draw the BER plot to reflect the transmission potential. Therefore, both phone and IoT devices we do many tests of different baud rate, all the way from the perfect transmission to the BER near or above 50\%. Regardless of the type of experiment, we do four tests for the same baud rate and record the results. Each test we transmit 100 bits of information. Four tests of one baud rate is a point on the BER diagram, we aim to restore the real BER diagram passing enough points of ASK and FSK in noise and without noise two situations.

\subsubsection{Related problems}

In our experiment, the results on IoT run very smoothly. However, we found an important issue in Android Phone which connects with the big.LITTLE processor technology. We do some contrast tests on the Samsung s7 phone to better analyze our APP. When there is no interference, everything happens as we expect. However, when we try the interference test which must cause heavier load in CPU, we find that the CPU load should raise but drops. 

So we conclude that we can use our program to complete covert communications on common multi-core phone, but for the phone which employs big.LITTLE technology, we can not complete our requirements temporarily. Because the magnitude of the CPU load is an important means of transmitting information regardless of ASK or FSK. When we add interference, the CPU load becomes smaller. This question we would address in the future and we focus on the common multi-core processor. But we still illustrate some background information about this technology to distinguish these two types of CPU.

To satisfy the demand that computing performance in mobile devices has grown at an incredible rate, A multi-core processor is a common architecture that a computer integrated circuit with two or more separate processing units, called cores. Multi-core processor increases overall speed for programs that support multithreading or other parallel computing techniques.  However, high performance requires fast CPUs which in turn can be difficult to fit in mobile power or thermal budget. At the same time battery technology has not evolved at the same rate as CPU technology. Therefore today we are in a situation where smartphones require higher performance, but the same power consumption. So ARM big.LITTLE technology has been designed to address these requirements. Big.LITTLE technology is a heterogeneous processing architecture which uses two types of processor. ”LITTLE” processors are designed for maximum power efficiency while ”big” processors are designed to provide maximum compute performance. Both types of the processor are coherent and share the same instruction set architecture (ISA). Using big.LITTLE technology, each task can be dynamically allocated to a big or LITTLE core depending on the instantaneous performance requirement of that task. Through this combination, big.LITTLE technology provides a solution that is capable of delivering the high peak performance demanded by the latest mobile devices, within the thermal bounds of the system, with maximum energy efficiency. 
\subsection{Decoding the data}
Whether it is FSK or ASK, all the CPU load information has been saved to the CSV file. In this section, we explain how to decode these files by Python to recover the original signals. Our main purpose is to explore the maximal potential of this communication method, so we may solve problems from ideal angle. 
\subsubsection{ASK decode}




==> sec_background.tex <==
\section{Background}
\label{sec:background}
In this section, we summarize the principal of CPU workloads in modern Android mobile phones and Android Things.
  
\subsection{Android CPU workloads}


\subsection{JavaScript and workloads}


\subsection{Workloads and CPU Frequency}


\subsection{DVFS and big.LITTLE}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> sec_motivation.tex <==
\section{Motivation}
\label{sec:motivation}

==> src/chirp.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(2484.00,1260.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2175,55){\makebox(0,0)[l]{\strut{}time}}%
      \put(365,1163){\makebox(0,0)[l]{\strut{}workload}}%
      \put(189,97){\rotatebox{90}{\makebox(0,0)[l]{\strut{}baseline}}}%
      \put(189,912){\rotatebox{90}{\makebox(0,0)[l]{\strut{}full}}}%
      \put(1209,-152){\makebox(0,0){\strut{}$T$}}%
      \put(2087,-152){\makebox(0,0){\strut{}$2T$}}%
      \put(769,55){\makebox(0,0){\strut{}bit 0}}%
      \put(1648,55){\makebox(0,0){\strut{}bit 1}}%
      \put(330,-152){\makebox(0,0){\strut{}0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chirp}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> src/chirp2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(2484.00,1260.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2175,55){\makebox(0,0)[l]{\strut{}time}}%
      \put(365,1163){\makebox(0,0)[l]{\strut{}workload}}%
      \put(189,97){\rotatebox{90}{\makebox(0,0)[l]{\strut{}baseline}}}%
      \put(189,912){\rotatebox{90}{\makebox(0,0)[l]{\strut{}full}}}%
      \put(1209,-152){\makebox(0,0){\strut{}$T$}}%
      \put(2087,-152){\makebox(0,0){\strut{}$2T$}}%
      \put(769,55){\makebox(0,0){\strut{}bit 0}}%
      \put(1648,55){\makebox(0,0){\strut{}bit 1}}%
      \put(330,-152){\makebox(0,0){\strut{}0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{chirp2}}%
    \gplfronttext
  \end{picture}%
\endgroup

